Disentangling Observed Causal Effects from Latent Confounders using Method of Moments

Discovering the complete set of causal relations among a group of variables is a challenging unsupervised learning problem. Often, this challenge is compounded by the fact that there are latent or hidden confounders. When only observational data is available, the problem is ill-posed, i.e. the causal relationships are non-identifiable unless strong modeling assumptions are made. When interventions are available, we provide guarantees on identifiability and learnability under mild assumptions. We assume a linear structural equation model (SEM) with independent latent factors and directed acyclic graph (DAG) relationships among the observables. Since the latent variable inference is based on independent component analysis (ICA), we call this model SEM-ICA. We use the method of moments principle to establish model identifiability. We develop efficient algorithms based on coupled tensor decomposition with linear constraints to obtain scalable and guaranteed solutions. Thus, we provide a principled approach to tackling the joint problem of causal discovery and latent variable inference.

==> motivation.tex <==
\section{A MOTIVATION EXAMPLE}


==> upload/analysis.tex <==
\vspace{-5pt}
\vspace{-5pt}
\vspace{-5pt}

\section{Recovery Guarantees}
\label{sec:analysis}

With the recovered response matrices, in this section, we analyze the correct recovery of the mixing matrix $\mathbf{A}$ and the observed causal matrix $\mathbf{B}$, with  interventions. All the proofs are in the Appendix. 

%both partial, or full ($\nn$)

Since the optimization in Algorithm \ref{alg:1} is non-convex, we analyze a variant of Algorithm \ref{alg:1}. This variant involves recovering 
each of $\mathbf{C}$ and $\mathbf{D}_i$ separately using tensor methods using Eq. \ref{eq:ica_tensor}, and finding a permutation on columns of $\mathbf{C}$ and $\mathbf{D}_i$ such that is minimizes the linear system \ref{eq:opt_1} - \ref{eq:opt_2}. 
\begin{align}
    \min_{\mathbf{C}} \| K_4(\mathbf{C}) - \mathbf{M}_4(\mathbf{X}) \|_F^2   , \hspace{1em}  \min_{\mathbf{D}_i}   \| K_4(\mathbf{D}_i) - \mathbf{M}_4(\mathbf{Y}_i) \|_F^2 \label{eq:ica_tensor}
\end{align} and using the recovered $\mathbf{C}$ and $\mathbf{D}_i$, we optimize the following
\begin{subequations}
\begin{align}
\label{eq:opt_1}
\min_{\mathbf{A},\mathbf{B}, \text{perm}(\mathbf{C}), \text{perm}(\mathbf{D}_i)} \ \  &  \left\|(\mathbf{I}-\mathbf{B})\mathbf{C}-\mathbf{A}\right\|_F^2 + \sum_{i=1}^{\nn} \left\|(\mathbf{I}-\mathbf{B}_i)\mathbf{D}_i-\mathbf{A}_i\right\|_F^2\\
\text{s.t. } \ \ & \mathrm{rank}\left(\mathbf{A}\right) = \min\{\nm,\nn\},
\qquad \mathbf{A}\in\mathbbm{R}^{\nn\times\nm},\label{eq:opt_2}
% 
\qquad\mathbf{B}\in\mathbbm{R}^{\nn\times\nn},
\end{align}
\end{subequations} where $perm(\cdot)$ represents permutation of the columns. Thus, we find an optimal permutation that minimizes (\ref{eq:opt_2}). The above optimization is computationally more expensive than Algorithm 1 since it requires search over all permutations. But it allows us to provide theoretical guarantees on recovery.

% Before proceeding to the identifiability results, we first consider necessary conditions on the number of interventions for our model.
\vspace{-1mm}
We   now provide theoretical guarantees for this variant. 
\subsection{Recovery with Infinite Samples }

%\textbf{With partial interventions.} First, we consider the case when only $k\leq\nn+1$ interventions are allowed and denote the set of interventions by $\{\mathcal{I}_i: i\in\mathcal{K}\}$ with $\mathcal{K}=k$. Suppose the values used in the interventions $\lambda_1,\ldots,\lambda_{\nn}\in\mathbbm{R}$ are arbitrary real numbers. 

We first analyze the case when infinite number of samples are available to the algorithm. In this case, the following theorem holds.
%
\begin{theorem}[Unique recovery with infinite samples]\label{thm:1} There exists a unique permutation of columns of  matrices $D_i$, recovered from tensor decomposition methods, such that $(\mathbf{I}-\mathbf{B}_i)\mathbf{D}_i=\mathbf{A}_i$ for all $i$.
The mixing matrix $\mathbf{A}\in\mathbbm{R}^{n\times m}$ and the observed causal matrix $\mathbf{B}\in\mathbbm{R}^{\nn\times \nn}$ are uniquely recovered under the assumptions that $\mathbf{A}$ has full column rank and $\mathbf{B}$ is strict lower triangular.\end{theorem}

%\textbf{With $\nn+1$ interventions.}
%As an implication of Theorem~\ref{thm:1}, when $\nn+1$ interventions are available, i.e., interventions can be done at each variable and passive observations are collected, the causal effects can then be recovered. Formally,
%the following corollary demonstrates the uniqueness of the recovered mixing matrix $\mathbf{A}$ and observed causal matrix $\mathbf{B}$ based on Algorithm~\ref{alg:1}. 

%\begin{corollary}
%\label{coro:1}
%Suppose the response matrices $\{\mathbf{D}_i:i=0,\ldots,\nn\}$ are correctly recovered such that the linear systems in Sec.\ref{sec:causal_effect} hold. The matrices $\mathbf{A}\in\mathbbm{R}^{n\times m}$ and $\mathbf{B}\in\mathbbm{R}^{n\times n}$ can be uniquely determined (up to permutation and scaling).
%\end{corollary}
% \tongxin{
% I restated the theorem as follows. 
%\begin{theorem}\label{thm:1}Suppose $0\in\mathcal{K}$ and the response matrices $\{\mathbf{D}_i: i\in\mathcal{K}\}$ are correctly recovered such that $(\mathbf{I}-\mathbf{B}_i)\mathbf{D}_i=\mathbf{A}_i$ for all $i\in\mathcal{K}$.The mixing matrix $\mathbf{A}\in\mathbbm{R}^{n\times m}$ and the observed causal matrix $\mathbf{B}\in\mathbbm{R}^{\nn\times \nn}$ can be uniquely determined.
% The rows $\{\mathbf{a}_i\in\mathbbm{R}^{m}:i\in\mathcal{K}\}$ of the mixing matrix $\mathbf{A}\in\mathbbm{R}^{n\times m}$ and the columns $\{\mathbf{g}^{(i)}\in\mathbbm{R}^{\nn}:i\in\mathcal{K}\}$ of $\mathbf{G}:=(\mathbf{I}-\mathbf{B})^{-1}\in\mathbbm{R}^{\nn\times \nn}$ can be uniquely determined (up to permutation and scaling).
%\end{theorem}
% }

% The proof is postponed to Appendix~\ref{append_a}.


\subsection{Recovery with Finite Samples}


We analyze the number of data samples, denoted by $N$, required in Algorithm~\ref{alg:1}. Suppose we have no prior information and the subroutine of tensor method is performed in an unsupervised manner\footnote{Similar argument holds for the semi-supervised ICA learning set-up in~\cite{pmlr-v28-anandkumar13}.}. To be consistent with the settings of Algorithm 1 in~\cite{JMLR:v15:anandkumar14b}, the $4$-th order moments $\mathbf{M
}_4$ with respect to the response matrices $\mathbf{C},\mathbf{D}_1,\ldots,\mathbf{D}_{\nn}$ are estimated empirically from $N$ observed measurements. We assume the following conditions for the theorem to hold:
%\noindent (1). Rank condition: $\nm$ is at most $O(\nn)$.

%\noindent (2). Matrices $\mathbf{C},\mathbf{D_1},\ldots,\mathbf{D}_{\nn}$  are selected uniformly i.i.d from a unit $\nn$-dimensional sphere.
\noindent (1). Matrix $\mathbf{A} $ has full column rank and $\mathbf{B}$ is strict lower triangular.
\noindent (2). The entries of $\mathbf{H}$ are independent sub-Gaussian variables with $\smash{\mathbbm{E}[H_j^2]=1}$ and the $4$-th order cumulant $\textbf{M}_4$  is non-zero.
\noindent (3). The number of samples satisfies $N\geq \widetilde{\Omega}\left(\nn\nm^6\right)$.
\noindent (4). The initialization is performed by 4-th order generalization of SVD-based technique, with the number of initializations as $\smash{L \geq \nm^{\Omega(\nm^2/\nn^2)}}$.
%\noindent (6). The signs of $\mathbf{A}$ and $\mathbf{B}$ are known.

% \begin{enumerate}
%     \item Rank condition: $\nm=\Theta(\nn)$.
%     \item The columns of $\mathbf{D}_0,\ldots,\mathbf{D}_{\nn}$ are selected uniformly i.i.d from a unit $\nn$-dimensional sphere.
%     \item The entries of $\mathbf{H}$ are independent sub-Gaussian variables with $\mathbbm{E}\left[H_j^2\right]=1$ and the $4$-th order cumulant $M_4$ defined in (\ref{eq:cumulant}) is non-zero.
%     \item The number of samples satisfies $N\geq \widetilde{\Omega}\left(\nn\nm^6\right)$.
%     \item The initialization is performed by 4-th order generalization of SVD-based technique, with the number of initializations as: $L \geq \nm^{\Omega(\nm^2/\nn^2)}$.
%     \item The signs of the original matrices $\mathbf{A}$ and $\mathbf{B}$ are known.
% \end{enumerate}
Consider the estimated matrices $\widehat{\mathbf{A}}$ and $\widehat{\mathbf{B}}$. Let $\widehat{\mathbf{G}}:=(\mathbf{I}-\widehat{\mathbf{B}})^{-1}$. The next theorem states that given the conditions in above, the $\infty$-norm error for the recovered rows of $\widehat{\mathbf{A}}$ and columns of $\widehat{\mathbf{G}}$ is bounded from above.
\begin{theorem}[Sample Complexity]
Suppose the above conditions (1)-(3) hold. Then the rows of the estimated mixing matrix $\widehat{\mathbf{A}}$ and the columns of the estimated observed causal matrix $\widehat{\mathbf{G}}$ given by Algorithm~\ref{alg:1} satisfy that for $i=1,\ldots,\nn$, with high probability, 
\begin{align*}
&\left|\left|\mathbf{a}_i-\widehat{\mathbf{a}}_i\right|\right|_{\infty}\leq O\left(\frac{\nm^2\max\{\nn,\nm\}^3}{\sqrt{\nm}\min\{N,\sqrt{\nn^3 N}\}}\right)
\qquad \left|\left|\mathbf{g}^{(i)}-\widehat{\mathbf{g}}^{(i)}\right|\right|_{\infty}\leq O\left(\frac{\nm^2\max\{\nn,\nm\}^3}{\sqrt{\nn}\min\{N,\sqrt{\nn^3 N}\}}\right),
\end{align*}
\label{thm_2}when sign ambiguity and column permutation are taken into account.
\end{theorem}



\vspace{-10pt}

% For poster

% \begin{theorem*}
% Under certain conditions and assuming the number of samples satisfies $N\geq \widetilde{\Omega}\left(\nn\nm^6\right)$, the rows of the estimated mixing matrix $\widehat{\mathbf{A}}$ and the columns of the estimated causal matrix $\widehat{\mathbf{G}}$ given by Algorithm~\ref{alg:1} satisfy that for $i=1,\ldots,\nn$, with high probability, 
% \begin{align*}
% &\left|\left|\mathbf{a}_i-\widehat{\mathbf{a}}_i\right|\right|_{\infty}\leq O\left(\frac{\nm^2\max\{\nn,\nm\}^3}{\sqrt{\nm}\min\{N,\sqrt{\nn^3 N}\}}\right),\\
% &\left|\left|\mathbf{g}^{(i)}-\widehat{\mathbf{g}}^{(i)}\right|\right|_{\infty}\leq O\left(\frac{\nm^2\max\{\nn,\nm\}^3}{\sqrt{\nn}\min\{N,\sqrt{\nn^3 N}\}}\right).
% \end{align*}
% \label{thm_2}
% \end{theorem*}

% The proof can be found in Appendix \ref{append_b}.


\subsection{Necessary Conditions on Interventions}

Consider interventions $\mathtt{Do}(X_i = \lambda_i)$ on the $\nn$ variables $X_1,\ldots,X_{\nn}$ denoted by  $\{\mathcal{I}_i: i\in \{0\}\cup\{1,\ldots,\nn\}\}$ where $\mathcal{I}_0$ is the null intervention of passive observations. The following necessary conditions on the number of interventions hold.

\begin{theorem}[Necessary conditions; SEM]
\label{thm:necessary}
There exists a graph $G=\left(\mathcal{X}\cup\mathcal{H},E\right)$ such that any collection interventions  $\{\mathcal{I}_i: i\in \mathcal{S}\}$ with $\max\{|\mathcal{S}|,m\}\leq \nn-1$ cannot recover its edge set $E$.
\end{theorem}

\begin{remark}
Our results indicate that even with an SEM model, if $m\leq \nn-1$, then the worst-case recovery of causal effects still requires $\nn$ interventions. In contrast, for graphical causal models with perfect data and faithfulness assumption similar to our Assumption~\ref{ass:1}, the authors of~\cite{Eberhardt2006} (see Proposition 2) have shown that $\nn-1$ interventions, counting the null intervention of passive observations (with each randomizing a single variable) are necessary to determine the causal relations of $\nn$ variables. 
% The proof can be found in Appendix~\ref{app:proof_of_thm_necessary}. 
\end{remark} 

\vspace{-5pt}




% \begin{remark}
% The theorem above concludes our identifiability results. With the help of $\nn+1$ interventions, if the  response matrices $\mathbf{D}_0,\ldots,\mathbf{D}_{\nn}$ are correctly recovered, the theorem implies that the causal effects represented by the matrices $\mathbf{A}$ and $\mathbf{B}$ can recovered.
% \end{remark}

% In the remaining part of this paper, we state a bound on the number of samples required for recovering   $\mathbf{A}$ and $\mathbf{B}$. 
\section{Simulation}

We validate Algorithm~\ref{alg:1} by showing the trade-offs of the number of samples used and the accuracy of recovery. We generate each $\mathbf{H}_k$ i.i.d. according to a Laplacian distribution with mean $1$ for $k=1,\ldots,m$ and each $\mathbf{X}_{i}$ i.i.d. according to a Gaussian distribution with mean $0$ and variance $1$ for $i=1,\ldots,\nn$. The noise vector $\mathbf{N}$ has i.i.d. Gaussian entries with mean $0$ and variance $10^{-3}$. Figure~\ref{fig:sample_complexitiy} depicts the sample complexity results for recovering the observed causal matrix. In particular, we generate data from a linear system with different numbers of observables and hidden variables. We restart the optimization 20 times to find the best optimization error. We plot the best recovery error on $\mathbf{B}$ using Algorithm \ref{alg:1} on different number of variables when there are same number of hidden variables and the observables (3 variables: Figure \ref{fig:sample_complexitiy} Left, 4 variables: Figure \ref{fig:sample_complexitiy} Middle, 5 variables: Figure \ref{fig:sample_complexitiy} Right, 10 variables: Figure \ref{fig:ablation} Left). We can see that the estimation error on $\mathbf{B}$ decrease fast with more samples. We also see that the recovery error increases with the number of the observables and hidden variables.
\begin{figure}[t]
 \setlength{\tabcolsep}{-5pt}
\begin{tabular}{ccc}
      \includegraphics[height=3.5cm]{img/erors1.png}&
      \includegraphics[height=3.5cm]{img/erors2.png}&
      \includegraphics[height=3.5cm, trim={1cm, 0cm, 0cm, 0cm},clip]{img/erors4.png}
    \end{tabular}
     \caption{Simulation results in 3 observable and 3 hidden ({\bf Left}), 4 observable and 4 hidden ({\bf Middle}) and 5 observable and 5 hidden ({\bf Right}). Trade-offs of the number of samples $N$ and Mean square error on $\mathbf{B}$. Note here the total number of samples are $(n+1)\times N$. Within the same mode, the error decrease fast with more samples. The recovery error increases with the number of the observables and hidden variables.}
    \label{fig:sample_complexitiy}
\end{figure}
\subsection{Ablation Study}
We conduct an ablation study on misspecified number of hidden variables and less number of interventions to see how robust our method is. Figure \ref{fig:ablation}(Middle) demonstrate that we can use less number of interventions to achieve similar empirical results. This indicates we only need small number of experiments instead of intervening on all the variables in practice. Figure \ref{fig:ablation} (Right) shows that when our model, in particular the number of latent variables, are slightly misspecified, our results are still quite robust. 
\begin{figure}[h]
 \setlength{\tabcolsep}{-5pt}
 \centering
\begin{tabular}{ccc}
      \includegraphics[height=3.5cm]{img/erors_rebuttal_3.png}&
      \includegraphics[height=3.5cm]{img/erors_rebuttal_1.png}&
      \includegraphics[height=3.5cm]{img/erors_rebuttal_2.png}
    \end{tabular}
     \caption{ {\bf Left}: Simulation result on 10 observation variables with different numbers of interventions. {\bf Middle}: Performance with increasing number of interventions with a 4-variable model. We can observe that we can use less intervention to achieve similar empirical results with full interventions. {\bf Right}: Performance with misspecified number of latent variables on a 3-variable model. We can see that the model is relatively robust to small perturbations on number of latent variables.}
    \label{fig:ablation}
    \vspace{-0.3cm}
\end{figure}

% to eliminate the ambiguity caused by scaling and permutation, we focus on the error defined below:
% \begin{align*}
%     \varepsilon:=\mathbbm{E}\left|\left|\mathbf{X}-\mathbf{A}\mathbf{H}-\mathbf{B}\mathbf{X}-\mathbf{N}\right|\right|_{2}
% \end{align*}
% where the expectation is taken over the randomness of $\mathbf{X}$, $\mathbf{H}$ and $\mathbf{N}$. 
% Note that $\mathbf{A}$ is permuted and having a small MSE on $\mathbf{B}$ 
% implies the recovered $\mathbf{A}$ and $\mathbf{B}$ satisfy the linear system in~\eqref{eq:1}. Our simulation demonstrates that the true mixing and observed causal matrices can be recovered using our method.



    


==> upload/conclusion.tex <==




% \section{CONCLUSION AND FUTURE WORK}
% \label{sec:conclusion}
% % {\color{red} experiment, non linear case, better intervention method, make this method practical(how to deal with like noise in tensor method)} \\
% In conclusion, we propose a novel approach to discover causal relation from experimental data based on recovering mixing and causal matrices in the latent linear structural equation model. We provide theoretical analysis regarding the conditions of unique identification and sample complexity for the method. 

% In the future, we plan to extend our theoretical results to cases with noisy data.
% An interesting extension of the methods is considering non-linear models including deep neural networks, where invariance of mixing matrices $\mathbf{A}$ does not hold in general but need to be enforced by constraints. We are also interested in relaxing the assumption of performing an intervention on each observable variable. By actively choosing the next intervention based on the performance from the last one, we expect to reduce the number of interventions and apply our method to more practical problems. Therefore, this work also paves the way to study off-policy learning and decision making in causal discovery. In reality, interventions are costly, making evaluating and optimizing interventions for more efficient causal discovery a promising future direction.


% \section{DISCUSSIONS}
% \label{sec:discussion}
% {\bf Potential applications.} Besides the recommendation system example, the framework proposed in this paper is general enough to apply to causal discovery in large power networks, social network analysis, and physical systems. In the social network case, an interesting subject is to study the causes for a user to tweet (retweet) in the \#MeToo movement. There are user features and behaviors as observable variables along with hidden variables that can be direct causes of both user feature variables and user behavior variables. Therefore, our approach provides huge opportunity in studying complex relations in large-scale systems\\
% {\bf In the small data region.} Latent variable extraction can be conducted in various ways. We propose to use method of moments when facing large-scale data. However, in the small data region, tensor decomposition can suffer from noises and errors. We could resort to other methods like joint factorization. Our general framework is compatible with different latent variable methods.\\
% % {\bf Adaptive intervention.} We plan to extend 
% {\bf When intervention changes the latent variables.} Another line of future work is to relax our assumption that latent variables are invariant during interventions. In this case, the model is augmented with an additional equation: $h = PX$, which captures how observable variables affect the hidden ones. This paper corresponds to the case when $P = O$. Our analysis and algorithm can be extended to more general cases after mild modification. We leave that to future research. 



\section{Conclusion and Discussion}
\label{sec:conclusion}
In this work, we propose a novel approach to discover causal relation from experimental data based on recovering mixing and causal matrices in the latent linear structural equation model. We provide theoretical analysis regarding the conditions of unique identification and sample complexity for the method. The effectiveness of our approach is validated by experiments.
An interesting extension of the methods is to consider non-linear models including deep neural networks, where invariance of a mixing matrix $\mathbf{A}$ does not hold in general but need to be enforced by constraints.
% We are also interested in relaxing the assumption of performing an intervention on each observable variable. By actively choosing the next intervention based on the performance from the last one, we expect to reduce the number of interventions and apply our method to more practical problems. 
% Therefore, this work also paves the way to study off-policy learning and decision making in causal discovery. In reality, interventions are costly, making evaluating and optimizing interventions for more efficient causal discovery a promising future direction.  
% Another line of future work is to relax our assumption that latent variables are invariant during interventions. In this case, the model is augmented with an additional equation: $h = PX$, which captures how observable variables affect the hidden ones. This paper corresponds to the case when $P = O$. Our analysis and algorithm can be extended to more general cases after mild modification. We leave that to future research. Below we present the academic and societal impacts of our work.

% {\bf Potential applications.}  
% {\bf In the small data region.} Latent variable extraction can be conducted in various ways. We propose to use method of moments when facing large-scale data. However, in the small data region, tensor decomposition can suffer from noises and errors. We could resort to other methods like joint factorization. Our general framework is compatible with different latent variable methods.


\newpage

% \section*{Broader Impact}
% Causal discovery is critical for scientific discovery, as well as social science research. By disentangling observable data from latent confounders, our approach can be applied to study complex relations in large-scale systems, such as power networks, genes networks, control systems and social networks wherein linear structural equation models are ubiquitous. The learned causal effects can be used for positive purposes that have direct societal impact, like developing drugs and treatment, behavior intervention for patients, and developing more efficient control systems. In the following we exemplify some representative application scenarios:

% \textbf{System identification of a power system.}

% Consider a radial distribution network in a power system. Our goal is to recover all the line parameters, such as impedance. Nodal measurements of a subset of the loads in the network are captured by sensing devices such as phasor measurement units (PMUs). Some of the loads, which however cannot be measured by the installed PMUs due to physical limitations and operational constraints, can be regarded as latent variables. In practice, it is often challenging to install metering devices to each individual non-utility generator or power plant. Traditional model-free statistical learning techniques for system identification of an unknown electricity grid with  unobserved loads requires a large amount of data. However, our approach enables a model-based recovery scheme. Given the measured phase angles by the PMUs, a swing equations-based model~\cite{talukdar2017learning} serves as a concrete realization of our generic linear structural equation model in~\eqref{eq:1}. Therefore our method has the potential to reduce sample complexity for system identification of a distribution network with latent nodes.

% \textbf{User behavior discovery in a social network}

% In the social network case, an interesting subject is to study the causes for a user to tweet (retweet) in the \#MeToo movement. There are user features and behaviors as observable variables along with hidden variables that can be direct causes of both user feature variables and user behavior variables. Our approach provides an opportunity in studying complex relations among users.

% On the other hand, our work requires interventions on variables, which calls for cautious implementation if the application is human-involved. In practice, our method should also work using fewer and soft interventions but more work still needs to be done. 


% In the social network and rec, an interesting subject is to study the causes for a user to tweet (retweet) and participate in public discussions. In physical networks, efficient system identification provide opportunity for fast learning and adaptation of the system. 
% There are user features and behaviors as observable variables along with hidden variables that can be direct causes of both user feature variables and user behavior variables. 
% The framework proposed in this paper is general enough to apply to causal discovery in large power networks, social network analysis, and physical systems. In the social network case, an interesting subject is to study the causes for a user to tweet (retweet) in the \#MeToo movement. There are user features and behaviors as observable variables along with hidden variables that can be direct causes of both user feature variables and user behavior variables. Therefore, our approach provides huge opportunity in studying complex relations in large-scale systems.
% We see no ethical issues related to this paper.  
% {\bf Adaptive intervention.} We plan to extend 



% \begin{itemize}
%     % \item 1. In potential applications, this framework proposed in this paper has close connection to network identification in power networks, social network analysis, and product-customer networks in recommendation system (in the partial intervention cases).  
%     % \item 2. ICA is not necessarily conducted by tensor methods, which requires large data.
%     % \item 3. This framework is also connected with factor models, where some of the factors are observed and some are not.
%     % \item 4. We can also extend the techniques to cases where observable variables can also affect latent confounders.
%     % \item 5. We can also extend to partial intervention
%     % \item 6. (Partial identifiability) Adaptive intervention \\
%     %     something like subspace result
    
% \end{itemize}


==> upload/intro.tex <==

\section{Introduction}

\label{sec:prev}
Discovery of causal relationships among a group of  variables lies at the heart of scientific discovery \cite{Pearl2009}. Inferring causes and effects, and separating them from spurious correlations, is central to scientific domains such as medical drug trials, high energy physics, and econometrics.  From a machine learning perspective, discovery of causal effects can lead to more robust, reliable, and interpretable predictions. 

Causal inference aims to learn strength of causal interactions on a known graph, while causal discovery also aims to learn the causal graph (and the parameters) from data. This problem is challenging especially in the presence of hidden or latent confounders, which make the problem ill posed. These are variables that are not directly observed but interact with the observables. These hidden variables cause spurious associations among the observed  variables and make it challenging to differentiate causal relations from spurious correlations. For instance, in drug trials, there are many unobserved factors that affect drug efficacy in a patient (e.g. their lifestyle choices), and not all of that is recorded.
% As another example, if we want to understand consumer behavior under online recommendations, there are many hidden factors that are not recorded. Moreover, privacy laws  further prevent collecting detailed and invasive information about the consumers.  On the other hand, companies may have large-scale information about  consumer and product features,  the history of consumer interactions and have the ability to carry out various experiments or interventions. 
As another example, to do system identification in physical systems, like control systems, not all the contributors to the dynamics are observed. This can be due to the difficulty in data collection or the limitations in data fieldity \cite{shi2019neural}. On the other hand, it is feasible to intervene or manipulate the physical system to record different kinds of data. Using such interventions to learn causal relationships is an interesting problem.
% The question is whether  we can use true underlying causes and effects that drive consumer behavior? 

%Disentangling the causal relations from confounding effects is the key to causal structure discovery.



%Throughout this paper, we use finding causes of consumer behavior in the recommendation system to motivate our modeling choices and assumptions. In order to discover the causes of customer behavior, we have customer features, product features, and recorded consumer behaviors available in the data as observational variables. However, there can be both observable and unobservable variables as direct common causes to the customer or product features and shopping behaviors. For example, we observe that red items are popular among Chinese customers. The season variable indicating the Spring Festival can be either observed or not. If not, we should infer the confounding effect of the season variable would avoid recommending unseasonal items to customers. 

% \aacomment{move figure 1 near summary of contributions}

% In many practical applications of empirical sciences, there exist variables that are unobserved but affect the visible factors in the model. 
%It is often impossible to uniquely identify the underlying causal relationships, when only observational data is available, unless strong modeling assumptions are made. Instead when interventions are available, 

The problem we consider is two-fold. We aim to simultaneously discover the relationships among a group of observed variables, and in addition, discover latent factors and their relationships with the observables. We aim  to solve both causal structure discovery and latent variable inference.

%\vspace{7pt}
%* Equal Contribution

\newpage
\paragraph{Causal Discovery with Interventions} While observational data is easy to obtain, causal relationships cannot always be uniquely identified using only observational data. 
%\cite
Interventions provide essential information for discovering the causal effects. For example, in structural equation models (SEMs)~\cite{Silva:2006:LSL:1248547.1248555}, the act of assigning a variable $X$ to a specific value $x$ allows us to dislodge $X$ from its prior causes and evaluate the expected change of other variables. More generally, softly intervening on a subset of variables induces a new probability distribution over the variables~\cite{Pearl2009}. This has been utilized previously  for estimating causal effects when the confounders are also observed variables~\cite{Pearl2009}. What we consider is the general interventional framework in this paper. Interventions are usually represented using $\mathbf{Do}$ operator. For example, in Figure \ref{fig:do}, $\mathbf{Do(X_1)}$ represents intervention on variable $X_1$. As a consequence, the incoming 
edge from $H$ to $X_1$ will be removed after the intervention.
\begin{wrapfigure}[9]{r}{0.45\textwidth}
% \vspace{-0.2in}
      \includegraphics[height=2.45cm, trim={4cm, 8cm, 9cm, 8cm},clip]{img/do_operator_1.pdf}
    \caption{The Do operator. }
    \label{fig:do}
\end{wrapfigure}
% \aacomment{cite}
% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=0.65\linewidth]{img/intervention.png}
%     \caption{Demonstration of intervention. }
%     \label{fig:sample_complexitiy}
% \end{figure*}


% With the accessibility of large scale observational data in modern machine learning applications, it is tempting to model unobserved confounders using latent variable models. % Although a plenty of work has been done on estimation of causal effects \cite{Hoyer:2008:ECE:1414098.1414341},\cite{10.1007/978-3-540-75256-1_4} using either background knowledge \cite{Chen:2016:IKS:3061053.3061120}, optimal interventions \cite{1606.05027}, etc,

%\vspace{-2mm}
\paragraph{Causal Discovery with hidden confounders}  Previous works that  focus on learning causal models with hidden confounding variables generally consider only  observational data ~\cite{hoyer2009nonlinear, zhang2012identifiability,1908.03932}.  However, these works  do not consider information obtained through interventions and hence, require strong modeling assumptions. Hence, they may not be applicable in many settings.  For instance, the linear, non-Gaussian, and acyclic model (LiNGAM) has been investigated for causal discovery using the independent component analysis (ICA) model under non-gaussian noise assumptions on observational data \cite{shimizu2006linear,shimizu2011directlingam}. It is recently extended to the hidden confounder 
setting\cite{1908.03932}. However, using observational data, it can only recover a class of causal models that are equivalent and compatible with observational data, but this does not guarantee unique identifiability of the causal relationships.

\paragraph{Latent variable models} In terms of latent variable modeling without causal relationships, there is a rich body of work proposing different classes of models and algorithms. We consider the independent component analysis (ICA) which assumes the presence of independent latent factors that mix together to generate the observed data~\cite{Hyvarinen:2000:ICA:351654.351659}. Learning the mixing process provides a natural  disentangled representation of the observed domain ~\cite{khemakhem2019variational}.
% \aacomment{cite NICA and VAE paper by Hyvarinen}. 
The simplest setting is when the mixing process is linear. In this case, the mixing matrix can be recovered provably and efficiently under mild assumptions using tensor decomposition methods and higher order (3rd or 4th) moments \cite{JMLR:v15:anandkumar14b}.
% \aacomment{cite anandkumar}. 

In contrast to tensor methods, standard approaches for learning latent variable models such as expectation maximization (EM) are not guaranteed to converge to the globally-optimal solution and are prone to failure in high dimensions. We consider the method of moments approach that  fits observed moments in order to estimate the model. For a wide class of   latent variable models that includes ICA, \cite{JMLR:v15:anandkumar14b} 
% \aacomment{cite anandkumar 2014 paper} 
showed that low order moments (up to third or fourth) is sufficient to provably learn the model. Efficient tensor decomposition algorithms have been developed that guarantee learning with polynomial sample and computational complexity. 

\paragraph{Our formulation} In this paper, we propose a new model termed as SEM-ICA that  combines the two frameworks, viz., linear SEMs and ICA, to incorporate both observables and latent confounders. We use a mixing matrix to represent the confounding effects between the latent variables and the observable variables. We use a DAG graph to represent the relationship among observable variables.  Thus, we assume a latent generative process, given by the  ICA model, and this acts as latent confounders to the causal discovery process among the observables. This is a reasonable assumption in many scenarios. For example, in power networks, our intervention on different distributors would not change the latent variables such as unrecorded weather or temperature.
% For example, in our recommendation system example, our interventions on recommending different products to different customers would not change the latent variables such as unrecorded user context or demographics.
% \aacomment{if u can come up with something  good keep it otherwise remove it}.

We assume that (soft) interventions are available and this helps disentangle the causal and latent effects. A key observation we make is the fact that there is invariance of the latent effects across different interventions, since we assume that they are driving the generative process of observations. This insight allows us to relate the data obtained  under different interventions. Our method generally allows for both hard interventions and soft interventions. But we focus our analysis and simulation on the hard interventions.
% \todo{(how about mentioning soft intervention?)}



%We make the following modeling assumptions, which enable us to analyze both latent confounders and causal effects among observational variables. First, we assume the latent variables are invariant under interventions, which means interventions would not change the value of the confounders. In our recommendation system example, our experiments on recommending different products to different customers would not change the latent variables such as seasons. Therefore, the relation between latent confounders and observable variables only changes for the intervened variables. We can then relate the shared property across multiple interventions. Second, given both observational and experimental data, we assume that the latent variables are independent with each other, which indicates that each step of latent variable extraction is an independent component analysis (ICAs)~\cite{Hyvarinen:2000:ICA:351654.351659} problem that recovers the mixing matrices. It is reasonable to have such assumptions in our recommendation example that unobservable confounders like seasons and economic cycles are independent.  Finally, we utilize the method of moments to discover latent variables. Thanks to recent advances in tensor methods, the efficiency of solving ICAs has been improved significantly~\cite{JMLR:v15:anandkumar14b}, which makes ICAs more tractable in large-scale data with performance guarantees. 


% should talk about method of moments as a way to discover latent variables

% However, previous work cannot focus on disentangling causal effects from confounding explicitly. For example, previous research covers methods that only recover a combination of causal and correlation relations using observational and experimental data ~\cite{Yoo:2012:BMC:2151204.2151412}. 
%We incorporate latent confounders in linear structural equation models (SEMs) and 
% However, the causal structure is in general not fully identifiable in the presence of latent variables using only observational data ~\cite{1908.03932}. %Previous works have mostly focused on learning models where all relations between variables are either correlation or causal. 
%consider causal discovery when intervention is possible. We use a mixing matrix and a causal matrix to represent the confounding effects and the causal relationship between observable variables, respectively. 
% The independence assumption between latent confounders is a reasonable one and there exist many situations where this assumption holds (such as situations similar to blind signal separation). 



%Our contributions are as follows:\\

\paragraph{Algorithmic Contributions} We establish a novel algorithm for learning linear SEM-ICA based on the method of moments. We consider moments computed both from observational and interventional data. In particular, each of these datasets can be expressed as another ICA model. Thus, we cannot hope to learn the correct underlying model by considering only observational data. In particular, we need to understand how the different datasets from different interventions are related to one another. We show that the mixing matrices of these models are related to the parameters of the underlying SEM-ICA model through a linear system of equations. We assume that the distribution of the generative latent factors is invariant under interventions. This holds in many cases when environmental conditions being invariant under controlled interventions. For example, in power networks, our intervention would not change the latent variables such as unrecorded weather or temperature.  We then formulate a joint optimization method that incorporates both the tensor decomposition and the linear systems with invariance constraints to obtain recovery of the mixing and observed matrices. 
% Combined with the formulated linear systems, we then establish the learning error guarantees for the whole algorithm.
% Our results show that the error of recovery the observed causal matrices converge quickly to zero.
\vspace{-5pt}


\paragraph{Theoretical Guarantees} We analyze a variant of our algorithm and prove  identifiability for the mixing and observed causal matrices. We demonstrate that under mild non-degeneracy conditions our method can identify both the mixing and observed causal matrices up to permutation, sign and scale. This requires the mixing matrix of the ICA model to be full-rank and the adjacent graph among observables to be directed acyclic graph(DAG). Both are natural for identifiability, which implies that the latent factors are not (linearly) degenerate.
 % Our identifiability is thus up to the permutation that matches latent factors of each ICA model. 
We also establish the learning error guarantees for the whole algorithm and show that we achieve polynomial sample and computational complexity. This is the first work that provides guaranteed causal discovery with hidden confounders.

\vspace{-5pt}
\vspace{-5pt}


%finding all permutations is not feasible and we



% The structure of the paper is as follows. In section \ref{sec:research}, we describe the problem setup, the model, and its notation. We further illustrate our method in section \ref{sec:ica} and \ref{sec:causal_effect}. We provide sample complexity analysis of our method in section \ref{sec:analysis}. Section \ref{sec:related} consist of related work. We conclude the paper and discuss further about future directions in section \ref{sec:conclusion}.

==> upload/methods.tex <==
\section{Problem Setup}
\label{sec:research}


\begin{figure}[t]
        \centering
        \setlength{\tabcolsep}{-5pt}
        \begin{tabular}{ccc}
          \includegraphics[height=4cm, trim={7cm, 6cm, 6.5cm, 6cm},clip]{img/sem_ica.pdf}&
           \includegraphics[height=4cm, trim={7cm, 6cm, 10cm, 6cm},clip]{img/ica.pdf}&
           \includegraphics[height=4cm, trim={7cm, 6cm, 10cm, 6cm},clip]{img/intervention.pdf} \\
           (a) & (b) & (c)
       \end{tabular}
       
         \caption{(a)  Graphical representation of the SEM-ICA model. The orange-circled nodes are the confounding variables that are mutually independent. The nodes in blue stand for observable variables and they are allowed to have causal relations between each other;
         (b) Graphical representation of the ICA model $\mathbf{X} = \mathbf{C}\mathbf{H}$. The coordinates of $\mathbf{H}$ are independent; (c) Graphical representation of the SEM-ICA model after intervene $i$th variable.}
        \label{fig:ICA}
     
    \end{figure}
% In this section, we formalize the model considered in this work, together with a brief summary of useful techniques. In the sequel, we present our model, which takes the confounding variables into consideration. The model is built upon the standard linear structural equation model~(SEM), with additional structural constraints.

% \subsection{Model and Notation}
\vspace{-5pt}
\vspace{-5pt}
Given a set of $\nn$ \textit{observable}  variables $\mathcal{X}:=\{X_1,\ldots,X_{\nn}\}$ and a set of $\nm$ \textit{confounding}  variables $\mathcal{H}:=\{H_1,\ldots,H_{\nm}\}$, we consider a directed graph $G=(\mathcal{X}\bigcup\mathcal{H},E)$ where $\mathcal{X}\cup\mathcal{H}$ is the vertex set. The edge set $E$ consists of all directed edges between vertices, which represent the causal relations between two neighboring variables. For a vertex $X\in\mathcal{X}$, the parent set of $X$ is denoted by $\mathrm{Pa}(X) \subseteq\mathcal{X}\bigcup\mathcal{H}$ such that $X' \in \mathrm{Pa}(X)$ if and only if there is a direct edge from $X'\in\mathcal{X}\bigcup\mathcal{H}$ to $X$. 
For modeling the causality among confounding variables and observable variables, we assume that the confounding variables are independent and there only exist paths from confounding variables to observable variables, but not the other way around. Moreover, we assume there is no self-loop and the partial graph with vertices in $\mathcal{X}$ is acyclic, whence can be regarded as a DAG. Therefore, the graph $G$ is a quasi-bipartite graph, as shown in Figure~\ref{fig:ICA} (a).


 We fix the notation for this paper. We use boldface letters $\mathbf{X}$ and $\mathbf{H}$ for random vectors and denote the $i$-th entry of $\mathbf{X}$ as $\mathbf{X}_i$. Observed measurements are realizations of $\mathbf{X}$, written as $\mathbf{X_{[1]}},\ldots,\mathbf{X_{[N]}}$ and $N$ is the number of samples. Matrices are denoted by uppercase boldface letters $\mathbf{A}$, $\mathbf{B}$, $\mathbf{C}$ and $\mathbf{D}$. For a matrix $\mathbf{A}$, the $i$-th row is written as $\mathbf{a}_i$ and the $i$-th column is denoted by $\mathbf{a}^{(i)}$. The $(i,j)$-th entry of $\mathbf{A}$ is denoted by $a_{i,j}$. The superscript $T$ refers to the transpose of a matrix or vector.



\subsection{Structural Equation Models with Latent Variables}

The set of observable variables is represented by $\mathbf{X}$ as a vector in $\mathbbm{R}^{\nn}$. The \textit{confounding (hidden) variables} are denoted by a vector $\mathbf{H}$ in $\mathbbm{R}^{\nm}$. We consider a linear model
% \footnote{Our model can be generalized straightforward to the noisy set-up. In particular, if a multivariate Gaussian noise $\mathbf{N}$ is added to the observations $\mathbf{X}$ such that $\mathbf{X}= \mathbf{A}\mathbf{H} + \mathbf{B}\mathbf{X} + \mathbf{N}  = \mathbf{C}\mathbf{H} + (\mathbf{I}-\mathbf{B})^{-1}\mathbf{N}$. Assuming the noise vector $\mathbf{N}\in \mathbbm{R}^\nn$ is a multivariate Gaussian random vector, then $(\mathbf{I}-\mathbf{B})^{-1}\mathbf{N}$ is also a multivariate Gaussian random vector that is independent of $\mathbf{H}$. Therefore, the tensor decomposition method proposed in \cite{JMLR:v15:anandkumar14b} can be applied to recover the matrix $\mathbf{C}$. See Theorem 3.4 in~\cite{JMLR:v15:anandkumar14b} and~\cite{comon2010handbook} for more details.} 
for the observable and confounding variables:
\begin{align}
\label{eq:1}
\mathbf{X} = \mathbf{A}\mathbf{H} + \mathbf{B} \mathbf{X} + \mathbf{N}
\end{align}
wherein $\mathbf{A}\in \mathbbm{R}^{\nn\times\nm}$ denotes the \textit{mixing matrix}. It represents the correlation between observable and confounding variables (and equivalently, the edges between confounding variables and observable variables in Figure \ref{fig:ICA}). Similarly, the matrix $\mathbf{B}\in\mathbbm{R}^{\nn\times\nn}$ is a \textit{observed causal matrix}, which encodes the causal relationship among observable variables (corresponding to directed edges in Figure \ref{fig:ICA}). Additive noise is written as $\mathbf{N}$.
Rearranging the terms, we obtain the following alternative expressions:
\begin{align}
\label{eq:2}
  \mathbf{X} = \mathbf{C}\mathbf{H} +\overline{\mathbf{N}}.
\end{align}
where $\mathbf{C}:=(\mathbf{I}-\mathbf{B})^{-1}\mathbf{A}$ and $\overline{\mathbf{N}}:=(\mathbf{I}-\mathbf{B})^{-1}\mathbf{N}$.
Here, $\mathbf{I}$ is an $\nn\times\nn$ identity matrix. Below we present the assumption of our model.
\begin{assumption}
\label{ass:1}
We assume that $\mathbf{A}$ is a full-rank matrix. We also suppose that the faithfulness assumption holds so that $a_{j,k}\neq 0$ if there is a causal path from $\mathbf{H}_k$ to $\mathbf{X}_j$ and $b_{i,j}\neq 0$ if there is a causal path from $\mathbf{X}_j$ to $\mathbf{X}_i$, for all $i,j=1,\ldots,\nn$ and $k=1,\ldots,\nm$.
\end{assumption}
With the help of $\nn$ interventions, we can discover the causal ordering of $X_1,X_2,...,X_n$ (see~(\ref{causal_order})). Hence after suitable permutation of the rows and columns of $\mathbf{B}$, we can formulate it as strict lower triangular and the matrix $\mathbf{C}$ is full-rank. In this work, we consider a new approach for identifying causal effects, \textit{i.e.,} recovering the mixing matrix $\mathbf{A}$ and observed causal matrix $\mathbf{B}$, by conducting interventions, defined in the next section.

\subsection{Interventions}

An intervention in causal discovery refers to the experiment that sets the values of the variables and isolates them from their causes. 

\begin{definition}
 {(\bf $\mathbf{Do}(\cdot)$ operator)}: We write $\mathbf{Do}(\cdot)$ as the intervention operator. Graphically, each ideal intervention $\mathbf{Do}(\mathbf{X}_i = \lambda_i)$  corresponds to removing all the directed edges from $\mathrm{Pa}(\mathbf{X}_i)$ to $X_i$ and set the coordinate $\mathbf{X}_i$ in $\mathbf{X}$ to be $\lambda_i$. We write $\mathbf{X}_i\in\mathbbm{R}^\nn$ as a vector with the $i$-th entry set to $\lambda_i$.

\end{definition} 
After an intervention $\mathbf{Do}(\mathbf{X}_i = \lambda_i)$, we assume $\mathbf{Y}_{-i} = \mathbf{X}_{-i} | \mathbf{Do}(\mathbf{X}_i = \lambda_i)$ and $Y_i = \lambda_i$,  the SEM defined in (\ref{eq:1}) still holds by modifying the mixing matrix and observed causal matrix as follow:
\begin{align}
\label{eq:intervened_system}
\mathbf{Y}_i = \mathbf{A}_i\mathbf{H} + \mathbf{B}_i\mathbf{Y}_i+ \mathbf{N}
\end{align}
where $\mathbf{A}_i$ and $\mathbf{B}_i$ are formed by setting the $i$-th rows of $\mathbf{A}$ and $\mathbf{B}$ as the all-zero vector and the unit vector $\mathbf{e}_i$. Rearranging the terms, similarly we obtain $\nn$ linear systems by intervening $\mathbf{Do}(\mathbf{X}_i = \lambda_i)$ for $i=1,\ldots,\nn$ and obtain the following alternative expressions:
\begin{align}
\label{eq:3}
  \mathbf{Y}_i = \mathbf{D}_i\mathbf{H}+ \overline{\mathbf{N}}_i, \ \text{ for } \ i=1,\ldots, \nn
\end{align}
where each matrix $\mathbf{D}_i:=(\mathbf{I}-\mathbf{B}_i)^{-1}\mathbf{A}_i\in\mathbbm{R}^{\nn\times\nm}$ is defined as the \textit{response matrix} to the intervention $\mathbf{Do}(\mathbf{X}_i = \lambda_i)$ and $\overline{\mathbf{N}}_i:=(\mathbf{I}-\mathbf{B}_i)^{-1}\mathbf{N}$. 
% In the next section, we will see that the observational data alone is not sufficient to recover the mixing and causal matrices of SEM-LV model. 

The goal of this work is to use both the observational data and the experimental data obtained by interventions $\mathbf{Do}(\mathbf{X}_i = \lambda_i)$ to identify the mixing matrix $\mathbf{A}$ and the observed causal matrix $\mathbf{B}$ in (\ref{eq:1}), under the assumption presented in Assumption~\ref{ass:1}.
In the following section, we discuss independent component analysis ( ICA) models and the associated tensor decomposition methods, that can be utilized for recovering the response matrices $\mathbf{C}, \mathbf{D}_1,\ldots,\mathbf{D}_{\nn}$, based on observed samples of $\mathbf{X}, \mathbf{Y}_{1},...,\mathbf{Y}_{\nn}$.

\subsection{Recovery of Causal Order} 
\label{causal_order}
It is well known that if single-variable interventions are conducted on the variables, causal ordering can be recovered \cite{hyttinen2012learning} \cite{Eberhardt2006}. Intuitively, by doing single-variable interventions, the causal ordering can be recovered by checking the variables that have changed after the interventions. Previous work provides method that can be used to recover the causal directions with $n-1$ interventions \cite{Eberhardt2006}. In our framework, we can recover the causal ordering immediately after getting the experimental data by doing interventions $\mathbf{Do}(\mathbf{X}_i=\lambda_i)$ on the variables $\mathbf{X}_1,\mathbf{X}_2,...,\mathbf{X}_n$. Furthermore, we can also determine matrices $\mathbf{A}$ and $\mathbf{B}$ using the same $n$ single-variable interventions as shown below. 

\section{Tensor Decomposition for ICA}
\label{sec:ica}

\subsection{Independent Component Analysis}




The classical independent component analysis (ICA) model is a well-known blind source separation method for separating a set of source signals from a set of mixed signals, with no or a little prior knowledge about the source signals or mixing process. ICA-based methods decompose a multivariate random signal into a set of independent non-Gaussian signals. Therefore, they can be applied to the linear structural equations in (\ref{eq:2}) and (\ref{eq:3}). Taking the equation in (\ref{eq:2}) as an example, our goal is to recover $\mathbf{C}$ whose columns are defined as \textit{independent components} (ICs), provided with data samples of $\mathbf{X}$. The corresponding graphical representation is depicted in Figure~\ref{fig:ICA}. 
The classical ICA problem is an ill-posed task since it has inevitable indeterminacy of permutation and dilation of the independent components. Therefore, without additional information, we can only recover columns of the matrix $\mathbf{C}$ in equation (\ref{eq:2}) up to permutation and scaling. Under Assumption~\ref{ass:1}, the matrix $\mathbf{C}$ in equation (\ref{eq:2}) is full-rank. Thus, it is identifiable if latent variables is non-Gaussian.


\subsection{Tensor Decomposition}
\label{sec:tensor}
Various techniques have been proposed to recover the factor matrix $\mathbf{C}$ of an ICA model $\mathbf{X}=\mathbf{C}\mathbf{H}+\overline{\mathbf{N}}$. In this work, we use the method in~\cite{JMLR:v15:anandkumar14b} for guaranteed recovery of ICs. This procedure, which we refer to as the \textit{tensor method}, uses higher-order moments of the random vector $\mathbf{X}$ to recover the columns of $\mathbf{D}$. Here, we use the $4$-th order cumulant of zero-mean vector $\mathbf{X}$ defined as:
\begin{align}
\label{eq:tensor}
    \mathbf{M}_4 = \mathbbm{E}\left[\mathbf{X}\otimes\mathbf{X}\otimes\mathbf{X} \otimes\mathbf{X}\right] - T 
\end{align}
where $T$ is the following $4$-th order tensor, $\text{ for } 1\leq i_1,i_2,i_3,i_4 \leq \nm$:
\begin{align*}
[T]_{i_1,i_2,i_3,i_4} =&\mathbbm{E}\left[\mathbf{X}_{i_1}\mathbf{X}_{i_2}\right]\mathbbm{E}\left[\mathbf{X}_{i_3}\mathbf{X}_{i_4}\right]
+\mathbbm{E}\left[\mathbf{X}_{i_1}\mathbf{X}_{i_3}\right]\mathbbm{E}\left[\mathbf{X}_{i_2}\mathbf{X}_{i_4}\right]
+\mathbbm{E}\left[\mathbf{X}_{i_1}\mathbf{X}_{i_4}\right]\mathbbm{E}\left[\mathbf{X}_{i_2}\mathbf{X}_{i_3}\right].
\end{align*}
%For general cases, if the mean of the $X_i$ is non-zero, we replace $\mathbf{H}_i$ by $\mathbf{H}_i-\mathbbm{E}[\mathbf{H}_i]$ in above. 
Denote by $\kappa_i$ the \textit{excess kurtosis}, a measure of non-Gaussianity
defined as
\begin{align}
\nonumber
% \kappa_i := \mathbbm{E}\left[(\mathbf{H}_i-\mathbbm{E}[\mathbf{H}_i])^4] - 3 \mathbb{E}[(\mathbf{H}_i-\mathbb{E}[\mathbf{H}_i])^2\right]^2,
\kappa_i := \mathbbm{E}\left[\mathbf{H}_i^4\right] - 3,
\end{align}
it follows that
% \begin{align}
% \label{eq:cumulant}
$\mathbf{M}_4 = \sum_{i=1}^{\nm}\kappa_i \mathbf{c}^{(i)}\otimes  \mathbf{c}^{(i)}\otimes  \mathbf{c}^{(i)}\otimes  \mathbf{c}^{(i)}$.
% \end{align}
The $4$-th order moment $\mathbf{M}_4$ can be estimated from observed measurements and tensor decomposition algorithms can be applied to recover the columns of $\mathbf{C}$. In particular, the alternating power updates proposed in~\cite{JMLR:v15:anandkumar14b} can be applied to solve the tensor decomposition problem in~(\ref{eq:tensor}).
\vspace{-5pt}
\section{Causal Effects Identification}
\label{sec:causal_effect}


%\subsection{Recovery of mixing and causal matrices}

Based on the causal ordering restored, the matrix $\mathbf{B}$ after suitable permutation of the rows and columns becomes a lower triangular matrix. Therefore, without loss of generality, we assume that $\mathbf{B}$ is strict lower triangular and thus matrix $\mathbf{C}$ is full-rank. 
% For notational convenience we let $\mathbf{A}_0:=\mathbf{A}$, $\mathbf{B}_0:=\mathbf{B}$, $\mathbf{D}_0:=\mathbf{C}$ and $\mathbf{X}_0:=\mathbf{X}$.  
The next step is to recover the mixing matrix $\mathbf{A}$ and observed causal matrix $\mathbf{B}$, from the linear systems:
% \begin{align}
% \label{eq:4.1}
 $(\mathbf{I}-\mathbf{B}_i)\mathbf{D}_i = \mathbf{A}_i, \quad \text{for } i=0,\ldots,\nn$, which is
% \end{align}
derived from (\ref{eq:3}) and (\ref{eq:2}). 

\subsection{Recovery of Response Matrices}
\label{PS_ind}
To obtain matrices $\mathbf{D}_0,\ldots,\mathbf{D}_\nn$ satisfying above, the labels of rows and columns of the matrices should be preserved, \textit{i.e.,} the rows and columns should correspond to the same confounding or observable variables. However, the tensor decomposition method reported in~\cite{JMLR:v15:anandkumar14b} leaves the permutation and scaling ({\textit{PS}}) for columns of any response matrix unknown. We name this issue {\textit {PS indeterminacy}}. Without considreation of time complexity, we can solve this issue in a brute force manner, by trying out different permutations of the hidden vectors since only the original mixing and observed causal matrices make the entire linear system solvable. Hence this issue will not affect the identification of our method. Also, heuristic ways exist for preserving the correspondence between columns of two response matrices $\mathbf{D}_i$ and $\mathbf{D}_j$ in practice. With prior knowledge, adding regularizers can also eliminate indeterminacy in an ICA model (\cite{lu2003eliminating}).

%\footnote{For instance, under the assumption that elements in $\mathbf{H}$ are distinct with each other, we can align the two hidden vectors $\mathbf{H}^{(1)}$ and $\mathbf{H}^{(2)}$, by doing the normalization, setting all the signs to be the same and sorting the two hidden vectors in an increasing order.}


\subsection{Recovery of Mixing and Observed Causal Matrices}

% For robust identification of $\mathbf{A}$ and $\mathbf{B}$, instead of solving the linear systems in (\ref{eq:4.1}), we can find the optimal solutions of the following least square optimization problem:
% \begin{subequations}
% \begin{align}
% \label{eq:opt_1}
% \min_{\mathbf{A},\mathbf{B}} \ \  &  \sum_{i=0}^{\nn} \left\|(\mathbf{I}-\mathbf{B}_i)\mathbf{D}_i-\mathbf{A}_i\right\|_2^2\\
% \text{s.t. } \ \ & \mathrm{rank}\left(\mathbf{A}\right) = \min\{\nm,\nn\},\\
% &\qquad \mathbf{A}\in\mathbbm{R}^{\nn\times\nm},\\
% \label{eq:opt_2}
% &\qquad\mathbf{B}\in\mathbbm{R}^{\nn\times\nn}.
% \end{align}
% \end{subequations}
% This optimization problem can then be solved using standard optimization tools like Gurobi and CVX.
For robust identification of $\mathbf{A}$ and $\mathbf{B}$, instead of solving the linear systems in section (~\ref{sec:causal_effect}), we combine the optimization objective in the tensor methods solving ICA with the linear systems to formulate a joint optimization objective: 
\begin{subequations}
\begin{align}
\label{eq:opt_1_1}
\min_{\mathbf{A},\mathbf{B}, \mathbf{C}, \mathbf{D}_i} \ \  & \left\|(\mathbf{I}-\mathbf{B})\mathbf{C}-\mathbf{A}\right\|_F^2  +  \sum_{i=1}^{\nn} \left\|(\mathbf{I}-\mathbf{B}_i)\mathbf{D}_i-\mathbf{A}_i\right\|_F^2 \\ &+ \| K_4(\mathbf{C}) - \mathbf{M}_4(\mathbf{X}) \|_F^2   + \sum_{i=1}^\nn \| K_4(\mathbf{D}_i) - \mathbf{M}_4(\mathbf{Y}_i) \|_F^2\\
\text{s.t. } \ \ & \mathrm{rank}\left(\mathbf{A}\right) = \min\{\nm,\nn\},
\quad \mathbf{A}\in\mathbbm{R}^{\nn\times\nm},\label{eq:opt_2_1}
% \label{eq:opt_2_1}
\quad\mathbf{B}\in\mathbbm{R}^{\nn\times\nn}.
\end{align}
\end{subequations}
Here, $K_4$ is the Kronecker product. In practice, we use Tensorly library \cite{kossaifi2019tensorly} to jointly optimize $\mathbf{D}_i$ together with $\mathbf{A}$ and $\mathbf{B}$. Specifically, the library utilizes the alternative least square (ALS) method for solving the optimization problems. In practice, we can also add regularization to match columns of $\mathbf{D}_i$ and $\mathbf{C}$ to eliminate the optimization difficulties brought by permutation. We outline the recovery process in Algorithm~\ref{alg:1}.

\begin{algorithm}[h]
%\hrule
%\hrule
\medskip
\KwData{Observed measurements (as copies of $\mathbf{X}$) and model parameters} %$\mathbf{x}^{(1)},\ldots,\mathbf{x}^{(N)}$\;
\KwResult{Estimated mixing and observed causal matrices $\widehat{\mathbf{A}}$ and $\widehat{\mathbf{B}}$}
\medskip
\hrule
\hrule
\medskip
\ {\it Step 1.} Recover the matrix $\mathbf{C}$ (using tensor decomposition methods).

\ {\it Step 2.} Obtain response matrices via interventions:
\For {$i = 1 \ to \ n $}{
 Perform the interventions $\mathbf{Do}$($\mathbf{X}_i$ = $\lambda_i$).
 
 Collect experimental measurements (as copies of $\mathbf{Y}_i$).
 
 Recover the response matrix $\mathbf{D}_i$ (using tensor decomposition methods).
}

\ {\it Step 3.} Recover causal ordering.

% \ {\it Step 4.} Conduct the elimination of \textit{PS} indeterminacy(see Section \ref{PS_ind}).

\ {\it Step 4.} Solve~\eqref{eq:opt_1_1}-\eqref{eq:opt_2_1}.

\Return{\text{Estimated $\widehat{\mathbf{A}}$ and $\widehat{\mathbf{B}}$}}
	\medskip
\caption{Algorithm for recovering mixing and observed causal matrices.}
\label{alg:1}
\end{algorithm}




==> upload/motivation.tex <==
\section{A MOTIVATION EXAMPLE}


==> upload/related.tex <==
\section{Related Work}
\label{sec:related}
% {\color{red} Most closely related work: kun zhang's work  \\
% https://arxiv.org/abs/1908.03932  \\
% https://arxiv.org/abs/1908.03932 \\
% } \\
{\bf Causal discovery without interventions: }
Traditionally, if the causal sufficiency assumption holds, \textit{i.e.,} no unobserved common causes exist for any pair of variables that are under consideration in the model, causal structure learning algorithms such as PC ~\cite{spirtes2000causation} and IC~\cite{Pearl2009} can identify a class of causal models that are equivalent to each other in terms of the conditional independence. Given more background knowledge, the models that fit the observed data can be narrowed down. 
% There are even cases when causal relation can be uniquely indentified~\cite{shimizu2006linear,shimizu2011directlingam} under the assumption that non-Gaussian distributions for the exogenous noise in the linear SEMs. 
In more general structure learning, assumptions about structures such as trees and polytress are made to learn from observational data \cite{sepehr2019algorithm,huangguaranteed}.
In this paper, we focus on modeling possible unobserved common causes, \textit{i.e.,} latent confounders, and establish a unique identification method using experimental data.  Utilizing hidden variables not only leads to a more descriptive representation of the model but also relaxes the computational complexity of many algorithms through dimensionality reduction. 
% There is a common concern in parameter learning for latent variable models is that there can be many (sometimes infinite) possible models that fit the same observational data due to unobserved effects. Thus, it is necessary to make some assumptions about hidden variables or the structure of the graphical model to make the identification process feasible \cite{pmlr-v28-anandkumar13}. 
% The closest work to this work is by Salehkaleybar et.al \cite{1908.03932}. They study the case of learning linear non-Gaussian causal models in the presence of latent variables. But they only use the observational data and they do not utilize the structure of the confounders to do causal discovery. 

{\bf Causal discovery using interventions:}
Studying causal discovery using interventions has a long history. There is a large body of work on experimental design for casual discovery based on combinatorics and search~\cite{eberhardt2007causation,eberhardt2007interventions, hyttinen2014constraint}. Representing the confounding effects implicitly and allowing multi-variable interventions, a linear cyclic causal model can be identified with presence of latent confounders~\cite{hyttinen2012learning}. Recent work focuses on developing efficient randomized algorithm to learn a causal graph with confounding variables in a minimal or constrained budget \cite{kocaoglu2017experimental,acharya2018learning,ghassami2017budgeted,ghassami2019interventional,hauser2012characterization,eaton2007exact,rothenhausler2015backshift}. Combined with active learning and optimization theory, interventions can be regarded as active data queries with different cost \cite{he2008active,addanki2020efficient}.
In our case, we assume the invariance of latent confounders to relate mixing matrices across interventions. We restrict to the case of single-variable intervention and learn the parameters of the mixing and causal matrices explicitly.

% {\bf Independent Component Analysis (ICA):} ICA Modeling has received much attention in the past two decades \cite{Hyvarinen:2000:ICA:351654.351659},\cite{book}. It is even possible to reduce the directed acyclic graph of a causal model to the bipartite graph of an ICA model \cite{pmlr-v28-anandkumar13}. Many techniques have been proposed to learn the parameter of an ICA model such as maximum likelihood estimation, minimization of mutual information, tensorial method, etc. \cite{JMLR:v15:anandkumar14b}, \cite{book}. In this paper, we use the alternating power updates tensor decomposition method presented in \cite{JMLR:v15:anandkumar14b} that is efficient and has guaranteed performance.

{\bf Causal inference and discovery with latent variable models:} Previous research on causal learning and latent variable models focus on the recovering the causal order \cite{tashiro2014parcelingam}. Lingam model has also been generalized to hidden variable cases \cite{hoyer2008estimation} and latent Gaussian confounders \cite{chen2013causality}. Recent study of causal inference using latent variable models \cite{wang2019blessings} assumes the conditional independence between observable variables given the latent confounders. It opens up a line of research about utilizing latent variables in regression problems for estimating the potential outcome. In contrast to that, our problem setting is a causal discovery one, where we recover both the causal relationships between observable variables together with the confounding effects.  


% \subsection{Our Contributions}
% Our contributions are summarized as follows.
% \begin{enumerate}
%     \item First, we tensor method
%     \item Second, identification result
%     \item Third, optimization method and sample complexity 
% \end{enumerate}

